A computational model for the evolution of learning physical micro-contents in peer instruction methodology

One of the most important active methodologies for physics learning developed in recent years is peer instruction. Its technique has allowed, among other things, to monitor students' conceptual learning. In this sense, \textcite{PhysRevSTPER.6.020105} has proposed a model that seeks to understand the dynamics of this methodology. However, her model is very phenomenological and overlooks fundamental aspects such as the cognitive process that students follow during interaction with their peers, the role of the instructor, the connection between content and student characteristics, and long-term learning. The objective of this thesis was to develop a computational model based on neurocognitive principles that aimed to address the shortcomings found in Nitta's work. The model was formulated, simulated, and validated based on several field studies on the learning of one-dimensional graphical interpretation and the falling of bodies among science and engineering students in Bogot\'a, Colombia

==> Appendices/Apen_binomial.tex <==
\chapter{Binomial}

A group of $N$ students is taking a test consisting of $n$ multiple-choice questions with only one answer and $s$ answer choices per question. The students are divided into two subgroups, where the $N_1$ students have a probability of $p_1$ to answer correctly each question, and the remaining $N-N_1$ students have a probability of $p_2$ to answer each question. Each student's response is modeled as a binomial distribution with $n$ trials and success probabilities $p_1$ and $p_2$, respectively. Do all $N$ students follow a single global binomial distribution in their answers?

Let $P_1$ and $P_2$ be the binomial distribution of each type of student and $P$ the global binomial distribution, which are given by
%------------
\begin{equation} \label{bino1}  %-
    P_1(k) = \binom{n}{k} p_1^k (1-p_1)^{n-k},
\end{equation}
%-----
\begin{equation} \label{bino2}  %-
    P_2(k) = \binom{n}{k} p_2^k (1-p_2)^{n-k}
\end{equation}
%----
and
\begin{equation} \label{binog}  %-
    P(k) = \binom{n}{k} p^k (1-p)^{n-k}
\end{equation}
%----

Based on the distribution's definition, we know that the probability of failure in each trial is $q_1=1-p_1$ 
and $q_2=1-p_2$, respectively. Now we put two conditions on the response probabilities:
\begin{equation} \label{ap_cod1}  %-
    p = a p_1+b p_2, 
\end{equation}
with $a$ and $b$ constant, that is, $p$ is a linear combination of $p_1$ and $p_2$. The other condition is:
\begin{equation} \label{ap_cod2}  %-
    a+b=1.
\end{equation}.

Substituting (\ref{ap_cod1}) in \ref{binog}, we find 
\begin{equation} \label{profin}  %-
    P(k) = \binom{n}{k} \left (a p_1+b p_2\right ) ^k (1-a p_1-b p_2)^{n-k}
\end{equation}
and since $\left (1-a p_1-b p_2  \right )=\left (a q_1+ b q_2  \right )$ then we  find
\begin{equation} \label{casfin}  %-
    P(k) = \binom{n}{k} \left (a p_1+b p_2\right ) ^k (a q_1+b q_2)^{n-k}, 
\end{equation}
since $q=a q_1+b q_2$.
\begin{equation} \label{tbino} 
(a q_1 + b q_2)^n = \sum_{k=0}^n \binom{n}{k} \left (a q_1 \right )^{n-k} \left (a q_1 \right )^k  
\end{equation}

==> resumen.tex <==
\chapter*{Resumen}
\thispagestyle{empty}
Una de las metodologías activas más importantes para el aprendizaje de la física desarrollada en los últimos años es la instrucción entre pares. Su técnica ha permitido, entre otras cosas, monitorear el aprendizaje conceptual de los estudiantes. En este sentido, \textcite{PhysRevSTPER.6.020105} ha propuesto un modelo que busca comprender la dinámica de esta metodología. Sin embargo, su modelo es muy fenomenológico y pasa por alto aspectos fundamentales como el proceso cognitivo que siguen los estudiantes durante la interacción con sus pares, el papel del instructor, la conexión entre el contenido y las características de los estudiantes y el aprendizaje a largo plazo. El objetivo de esta tesis fue desarrollar un modelo computacional basado en principios neurocognitivos que pretendía abordar las deficiencias encontradas en el trabajo de Nitta. El modelo fue formulado, simulado y validado con base en varios estudios de campo sobre el aprendizaje de la interpretación gráfica unidimensional y la caída de cuerpos en estudiantes de ciencias e ingeniería en Bogotá, Colombia.

Palabras clave: modelo computacional, instrucción entre pares, aprendizaje de la física, principios neurocognitivos, interpretación gráfica, unidimensional, caída delos cuerpos.
